'Simulacrum of Stories': Examining Large Language Models as Qualitative Research Participants

The recent excitement around generative models has sparked a wave of proposals suggesting the replacement of human participation and labor in research and development--e.g., through surveys, experiments, and interviews--with synthetic research data generated by large language models (LLMs). We conducted interviews with 19 qualitative researchers to understand their perspectives on this paradigm shift. Initially skeptical, researchers were surprised to see similar narratives emerge in the LLM-generated data when using the interview probe. However, over several conversational turns, they went on to identify fundamental limitations, such as how LLMs foreclose participants' consent and agency, produce responses lacking in palpability and contextual depth, and risk delegitimizing qualitative research methods. We argue that the use of LLMs as proxies for participants enacts the surrogate effect, raising ethical and epistemological concerns that extend beyond the technical limitations of current models to the core of whether LLMs fit within qualitative ways of knowing.

==> Sections/Acknowledgements.tex <==
\section{Acknowledgements}

==> Sections/Limitations.tex <==
\section{Limitations}

We acknowledge a few limitations in this work. Our participants were primarily academics with prior training in qualitative methods, which may not represent the diversity of perspectives or incentives outside of academic settings. Our study was conducted exclusively in English and involved researchers based primarily in the U.S. This limits the exploration of how cultural differences might influence the use of LLMs in qualitative research, particularly in non-English speaking or culturally diverse contexts. The study focused on a limited range of research topics, driven by the specific interests of our participants, which may not represent the full spectrum of qualitative research areas. The recruitment methods (social networks, email, institutional forums) may have introduced a selection bias, attracting participants who might already have preconceived notions about using LLMs in qualitative research. 

Another limitation relates to model selection and persona creation. We did not experiment with different language models; instead, we focused solely on GPT-4 from OpenAI, which is a closed-source model. This decision allowed us to maintain consistency across interviews, but it also means that our findings may not generalize to interactions with other LLMs that might respond differently under similar conditions. We did not fine-tune the LLM for specific personas, nor did we provide participants with extensive training on how to craft these personas. While this was an intentional choice to observe how researchers naturally engage with LLMs, it likely limited the variety and depth of the personas that were created. Participants were given limited time to develop their personas, which might have affected the richness of the LLM-generated data. 
% only explored text generation models, not multi-modal models
